Multi-Dimensional Ability Diagnosis for Machine Learning Algorithms

Machine learning algorithms have become ubiquitous in a number of applications (e.g. image classification). However, due to the insufficient measurement of traditional metrics (e.g. the coarse-grained Accuracy of each classifier), substantial gaps are usually observed between the real-world performance of these algorithms and their scores in standardized evaluations. In this paper, inspired by the psychometric theories from human measurement, we propose a task-agnostic evaluation framework Camilla, where a multi-dimensional diagnostic metric Ability is defined for collaboratively measuring the multifaceted strength of each machine learning algorithm. Specifically, given the response logs from different algorithms to data samples, we leverage cognitive diagnosis assumptions and neural networks to learn the complex interactions among algorithms, samples and the skills (explicitly or implicitly pre-defined) of each sample. In this way, both the abilities of each algorithm on multiple skills and some of the sample factors (e.g. sample difficulty) can be simultaneously quantified. We conduct extensive experiments with hundreds of machine learning algorithms on four public datasets, and our experimental results demonstrate that Camilla not only can capture the pros and cons of each algorithm more precisely, but also outperforms state-of-the-art baselines on the metric reliability, rank consistency and rank stability.

==> section/method.tex <==
% \section*{\emph{Camilla}: Task-Agnostic Cognitive Diagnostic Framework for Machine Learning Evaluation}

% \section*{Problem Definition}
% \section*{Preliminary and Problem Definition}

\section*{Materials and Methods}

Inspired by the psychometric theories from human measurement~\cite{newell1972human,nichols2012cognitively}, we propose a general diagnostic framework \emph{Camilla} for evaluating machine learning algorithms. For better illustration, we start with \emph{Camilla-Base}, a basic  version of \emph{Camilla} which uses classic MIRT~\cite{reckase2009multidimensional} as the backbone and incorporates explicit sample-skill mapping~\cite{tatsuoka1995architecture} to measure the \emph{Ability} of learners on explicit skills. Then, we augment this basic diagnoser with latent sample \emph{skill mask} factors and a multi-layer perception~(MLP) to accommodate most various machine learning tasks where the sample-skill matrix is unknown, without loss of precision and interpretability for capturing the interactions between learners and samples. Figure~\ref{Fig.camilla}A and Figure~\ref{Fig.camilla}B illustrate the schematic overview of \emph{Camilla-Base} and \emph{Camilla}. In the following of this section, we will introduce the workflows, training target, computation of the overall ability value and the implementation details of \emph{Camilla}s, respectively.



% What follows is a outline of three key components~(i.e. input, mapping layer and interaction layer) in \emph{Camilla}s, and we present the difference between \emph{Camilla-Base} and \emph{Camilla} in the following description.

\noindent\textbf{Camilla-Base.}~\emph{Input.} The input of \emph{Camilla-Base} includes the response logs/matrix $R$ from different well-trained learners to data samples, a pre-defined sample-skill matrix $Q$, and the representations of learners and samples.

\noindent 1)~\emph{Learner representation.} In this work, we focus on the \emph{Ability} assessment of individual learners. Therefore, we represent learner $s_i$ input as one-hot vector $s_i \in \{0, 1\}^{1\times N}$.

% and pay no attention on the inner architecture influence on the learner performance

% \noindent\textbf{2)~Sample representation.} Previous diagnosers mostly represent items~(e.g. exercise) independently with one-hot vector in various cognitive diagnosis tasks. As for cognitive diagnosis toward machine learning tasks, we argue that the representation of samples can benefit from unsupervised pre-trained methods. A mass of unsupervised pre-trained methods provides rational and abundant representations of samples, such as DeeperCluster~\cite{caron2019unsupervised} for images and BERT~\cite{DBLP:conf/naacl/DevlinCLT19} for text. These methods enable similar samples to have similar representations and make a great success in the downstream tasks. We consider that the performance of learners on the untried samples is similar to the similar tried samples and hence we represent sample $e_j$ with pre-trained feature $\widetilde{e_j} \in \mathbb{R}^{1\times D}$, where $D$ is the dimension of pre-trained feature. Generally, for tasks without pre-trained methods, we represent sample $e_j$ input as one-hot vector $\hat{e_j} \in \{0, 1\}^{1\times M}$ conventionally. For convenience, we represent the sample $e_j$ as $E_j \in \{\widetilde{e_j}, \hat{e_j}\}$, which line with these two circumstances.

\noindent 2)~\emph{Sample representation.} Similar to learner representation, we use one-hot vector $e_j \in \{0, 1\}^{1\times M}$ to represent sample $e_j$.


\noindent\emph{Mapping layer.} The mapping layer consists of factors that characterize the latent trait of learners and samples.

% \noindent\textbf{1)~Learner Ability.} The meaning of multidimensional \emph{Ability} factor is given in Definition~\ref{def:ability}. When explicit $Q$ matrix exists, each dimension of \emph{Ability} corresponds to the proficiency of learners on a specific skill. Otherwise, the dimension of learner \emph{Ability} factor is a hyperparameter. We characterize the \emph{Ability} factor $A_i$ of learner $s_i$ as follows:
% \begin{equation}
%     \small
%     A_i = \text{sigmoid}(s_i  \times  W_{A}),~ A_i\in (0, 1)^{1\times K}, W_{A}  \in \mathbb{R}^{N \times K}.
% \end{equation}

\noindent 1)~\emph{Learner Ability.} The meaning of multidimensional \emph{Ability} factor is given in Definition~\ref{def:ability}. Each dimension of \emph{Ability} corresponds to the proficiency of learners on a specific skill. We characterize the \emph{Ability} factor $A_i$ of learner $s_i$ as follows:
\begin{equation}
    A_i = s_i  \times  W_{A},
\end{equation}
where $A_i\in \mathbb{R}^{1\times K}$, $W_{A} \in \mathbb{R}^{N \times K}$ is a trainable transformation matrix, $K$ is the number of explicit skills pre-defined in the sample-skill matrix $Q$. During implementations, we can fix each value of $A_i$ into the range of $[0, 1]$, e.g. via Sigmoid function. 

%where $A_i\in (0, 1)^{1\times K}$, $W_{A}  \in \mathbb{R}^{N \times K}$.

\noindent 2)~\emph{Sample factor.} The sample factors characterize the latent trait of samples. In this paper, we assume the sample factors consist of three components: \emph{skill mask} factor, \emph{difficulty} factor and \emph{discrimination} factor.

% \noindent 1)~\emph{Sample skill mask factor.} As the proficiency of learners are characterized by a multi-dimensional factor, we consider that each sample focuses on different dimensions of learner \emph{Ability} factor, which can be evidenced by the sample-skill matrix $Q$. Specifically, the \emph{skill mask} factor depicts the skills that are most needed for a correct prediction of the sample and masks the other unrelated skills. If an explicit $Q$ exists, the \emph{skill mask} factor $Q_j$ of sample $e_j$ is fixed as:

\noindent (1)~\emph{Sample skill mask factor.} As the proficiency of learners are characterized by a multi-dimensional \emph{Ability}, we consider that different samples correspond to different dimensions of the learner \emph{Ability} factor, which can be evidenced by the sample-skill matrix $Q$. Specifically, the \emph{skill mask} factor depicts the skills that are most needed for a correct response of the sample by masking the other unrelated skills. The \emph{skill mask} factor $Q_j$ of sample $e_j$ is fixed as:
\begin{equation}
     Q_j = e_j  \times  Q,
\end{equation}
where $Q_j\in \{0, 1\}^{1\times K}$, $e_j$ denotes the one-hot vector of sample $e_j$. 

% Otherwise, we characterize the\emph{ skill mask} factor as a learnable factor with representation $E_j$ of sample $e_j$:
% \begin{equation}
%     \small
%     Q_j = \text{softmax}(E_j  \times  W_{Q}),
% \end{equation}
% where $Q_j \in (0, 1)^{1\times K}$, $E_j \in \{\widetilde{e_j}, \hat{e_j}\}$ and $W_Q$ is a trainable transformation matrix.

\noindent (2)~\emph{Sample difficulty factor.} Similar to curriculum learning~\cite{bengio2009curriculum} and self-paced learning~\cite{kumar2010self}, which suggest that there are differences between the difficulty of samples, we also argue that the \emph{difficulty} factor of samples should be taken into account in the learner \emph{Ability} assessment. Specifically, if one learner can correctly respond to a data sample while other learners cannot, then this sample with high \emph{difficulty} should contribute more to this learner's corresponding \emph{Ability}, and vice versa. Therefore, capturing the relationship between the \emph{Ability} factor of learners and the \emph{difficulty} factor of samples can help to more precisely predict how sure the learner can respond to the sample correctly. Following the classic MIRT\cite{reckase2009multidimensional}, the \emph{difficulty} factor of sample $e_j$ is represented as:
\begin{equation}
    D_j = e_j  \times  W_{D},
\end{equation}
where $D_j\in \mathbb{R}$, $e_j$ is the one-hot representation of sample $e_j$, and $W_D$ is a trainable transformation matrix.

\noindent (3)~\emph{Sample discrimination factor.} Following the psychometrics~\cite{lord1952theory}, sample \emph{discrimination} factor indicates the capability of sample $e_j$ to differentiate the mastery degree of learners. We represent the sample \emph{discrimination} factor as:
\begin{equation}
    b_j = e_j  \times  W_{b},
\end{equation}
where $b_j\in \mathbb{R}^{1\times K}$, and $W_{b}  \in \mathbb{R}^{M \times K}$ is a trainable transformation matrix.

\noindent\emph{Interaction layer.} After giving the input and mapping representation, the way to define a function for modeling the complex interactions among learners, samples and skills is one of the most important components for a diagnoser. Inspired by MIRT~\cite{reckase2009multidimensional}, we adopt an interaction layer which  outputs the probability $r_{ij}\in R$  that the learner $s_i$ responds to the sample $e_j$ correctly via the comparison between the multi-dimensional learner \emph{Ability} $A_i$ and the \emph{difficulty} $D_j$ of the sample in covered skills. In this layer, we define the diagnose function as (i.e. Eq.(\ref{equ:Camilla-Base})):
\begin{equation}
    p\left(r_{i j}=1|A_i, Q_j, b_j, D_j\right)=\frac{1}{1+e^{-Q_j \otimes b_j \cdot\left(A_i-D_{j}\right)}},
    \label{equ:Camilla-Base-2}
\end{equation}
where $\otimes$ is element-product and $\cdot$ is dot-product.

\noindent\textbf{Camilla.}~\emph{Input}.~For general applications in various machine learning tasks where the sample-skill matrix $Q$ may not be available, \emph{Camilla} takes only the response logs/matrix $R$ and the representations of learners and samples as input, and the definitions of learner and sample representations are the same as \emph{Camilla-Base}.

\noindent\emph{Mapping layer.} In the mapping layer of \emph{Camilla}, the principles of learner and sample factors inherit from \emph{Camilla-Base}. However, \emph{Camilla} utilizes a multi-layer perception (MLP), instead of the simplified
equation Eq.(\ref{equ:Camilla-Base-2}) in \emph{Camilla-Base}, to more precisely capture the interactions between learners and samples, and we revise the implementation of each factor to accommodate the general applications of \emph{Camilla}.

\noindent 1)~\emph{Learner Ability.}~To enhance the capability of MLP, the \emph{Ability} $A_i^{'}$ of learner $s_i$ are rescaled to [0, 1] via Sigmoid function:
\begin{equation}
    A_i^{'} = \text{Sigmoid}(s_i  \times  W_{A}^{'}),
\end{equation}
where $A_i^{'}\in (0, 1)^{1\times K^{'}}$, $W_{A}^{'} \in \mathbb{R}^{N \times K^{'}}$, and the dimension $K^{'}$ is a hyperparameter. 

\noindent 2)~\emph{Sample factors.}~Since there are various machine learning tasks where the sample-skill matrix $Q$ may be not explicitly accessible, we characterize the \emph{skill mask} factor $Q_j^{'}$ as a learnable factor for the representation of sample $e_j$:
\begin{equation}
    Q_j^{'} = \text{Softmax}(e_j  \times  W_{Q}^{'}),
\end{equation}
where $Q_j^{'}\in (0, 1)^{1\times K^{'}}$, $e_j$ denotes the one-hot vector of sample $e_j$, and $W_{Q}^{'}$ is a trainable
transformation matrix. The value of $Q_j^{'}$ in each dimension indicates the degree to which the sample $e_j$ is associated with each latent skill. In order to more precisely diagnose multidimensional \emph{Ability}, we characterize the latent traits of samples with multidimensional \emph{difficulty} factor $D_j^{'} \in (0, 1)^{1 \times K^{'}}$ and unidimensional \emph{discrimination} factor $b_j^{'}\in (0, 1)$. $D_j^{'}$ indicates the sample difficulty in each latent skill and has a one-to-one correspondence with the multifaced learner \emph{Ability} $A_i^{'}$. We obtain them by:
\begin{equation}
    D_j^{'} = \text{Sigmoid}(e_j  \times  W_{D}^{'})~~\text{and}~~b_j^{'} = \text{Sigmoid}(e_j  \times  W_{b}^{'}),
\end{equation}
where $W_{D}^{'} \in \mathbb{R}^{M \times K^{'}}$ and $W_{b}^{'} \in \mathbb{R}^{M \times 1}$ are trainable.

\noindent\emph{Interaction layer.} After giving the input and mapping representation, the way to define a function for modeling the complex interactions among learners, samples and the skills is one of the most important components for a diagnoser. Inspired by the cognitive diagnosis models in psychometric
theories~\cite{lord1952theory,wang2020neural}, we adopt an interaction layer which can combine cognitive diagnosis assumptions and neural networks for keeping both effectiveness and interpretability in machine learning evaluation. Specifically, the interaction layer outputs the probability $r_{ij} \in R$  that the learner $s_i$ responds to the sample $e_j$ correctly via the comparison between the multi-dimensional learner \emph{Ability} $A_i^{'}$ and the \emph{difficulty} $D_j^{'}$ of the sample in covered skills. In this layer, we first define the diagnose function as:
\begin{equation}\label{equ:Camilla}
     {Y}_{ij} = Q_j^{'} \otimes(A_i^{'} - D_j^{'}) \times b_j^{'},
\end{equation}
where $Y_{ij} \in  \mathbb{R}^{1\times K^{'}}$, $\otimes$ is element-product and $b_j$ is sample \emph{discrimination}. Then, we aggregate $Y_{ij}$ with a fully connected multi-layer perception (MLP) as follows:
\begin{equation}
\label{interaction_layer}
o = \text{sigmoid}(W_1Y_{ij} + b_1),~~
r_{ij} = \text{sigmoid}(W_2o + b_2).
\end{equation}

Following the solution of NeuralCD\cite{wang2020neural} in human performance
measurement, we also promise
the monotonicity in Assumption \ref{Ass:Mono} by normalizing the MLP where the parameters are restricted to be non-negative.

% \noindent\emph{Interaction layer.} After giving the input and mapping representation, the way to define a function for modeling the complex interactions among learners, samples and the skills is one of the most important components for a diagnoser. Inspired by the cognitive diagnosis models in psychometric
% theories~\cite{lord1952theory,wang2020neural}, we adopt an interaction layer which can combine cognitive diagnosis assumptions and neural networks for keeping both effectiveness and interpretability in machine learning evaluation. Specifically, the interaction layer outputs the probability $r_{ij}$  that the learner $s_i$ responds to the sample $e_j$ correctly via the comparison between the multi-dimensional learner \emph{Ability} $A_i$ and the \emph{difficulty} $D_j$ of the sample in covered skills. In this layer, we first define the diagnose function as:
% \begin{equation}
%     \small
%      {Y}_{ij} = Q_j \otimes(A_i - D_j) \times b_j,
% \end{equation}
% where $Y_{ij} \in  \mathbb{R}^{1\times K}$, $\otimes$ is element-product and $b_j$ is sample \emph{discrimination}. Then, we aggregate $Y_{ij}$ with a multi-layer perception as following:
% \begin{equation}
% \small
% \label{interaction_layer}
% %\begin{split}
% o = \text{sigmoid}(W_1Y_{ij} + b_1),~~
% r_{ij} = \text{sigmoid}(W_2o + b_2).
% %\end{split}
% \end{equation}



% To guarantee the monotonicity in Assumption~\ref{Ass:Mono}, we adopt a strategy which restricts weights of multi-layer perception~(e.g. $W_1$ and $W_2$) to be positive~\cite{wang2020neural}. It can be easily proved that $\frac{\partial r_{ij}}{\partial A_{ik}}$ is non-negative for each dimension \emph{Ability} $A_{ik}$ in $A_i$. Thus the monotonicity assumption is always satisfied during training.



\noindent\textbf{Diagnoser training.}
The loss function of diagnosers depends on the specific type of machine learning task. For instance, the cross entropy between prediction probability $\hat{r}_{ij}$ and the ground truth response of the learner $r_{ij}$ can serve as the loss function $\mathcal{L}_{\text{cls}}$ for classification learners\footnote{For instance, $r_{ij}=1$ represents the learner classifies the sample correctly (no matter the class labels of the sample), and 0 otherwise.}. As for regression tasks, we select the mean squared error as loss function $\mathcal{L}_{\text{reg}}$.
\begin{equation}
    \begin{split}
    \mathcal{L}_{\text{cls}}&=-\frac{1}{N}\frac{1}{M}\sum\limits_{i=1}^N\sum\limits_{j=1}^M\left(\hat{r}_{ij} \log r_{ij}+\left(1-\hat{r}_{ij}\right) \log \left(1-r_{ij}\right)\right), \\
    \mathcal{L}_{\text{reg}}&=\frac{1}{N}\frac{1}{M}\sum\limits_{i=1}^N\sum\limits_{j=1}^M \left(\hat{r}_{ij} - r_{ij}\right)^2.
    \end{split}
\end{equation}

With this loss function and the observed input data (e.g. $R$), both the multi-dimensional \emph{Ability} of learners and the factors (e.g. \emph{difficulty} and \emph{discrimination}) of samples can be estimated after inferring \emph{Camillas}. 

% \begin{equation}
%     \small
%     \mathcal{L}_{\text{cls}}=-\sum_{i}\nolimits\left(\hat{y}_{i} \log y_{i}+\left(1-\hat{y}_{i}\right) \log \left(1-y_{i}\right)\right).
% \end{equation}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{Figures/aggregate_ability_3.pdf}
    \caption{An example for the way of getting the specific proficiency from the learner to a subset of samples with \emph{Camilla}.}
    \label{Fig.compare}
\end{figure*}

\noindent\textbf{Computation of the overall ability value for each learner.}~In the foregoing, we show the way to output the multi-dimensional \emph{Ability} for each learner based on \emph{Camilla-Base} and \emph{Camilla}, respectively. Considering that it is also necessary to get the overall ability in some applications (e.g. Figure~\ref{Fig.COR}), we then give the solution for summarizing a unidimensional ability value of each learner from this \emph{Ability} vector.


\noindent\emph{Camilla-Base.}~\emph{Camilla-Base} exploits the explicit sample-skill matrix to get the \emph{skill mask} factors of data sample, and the multi-dimensional \emph{Ability} $A_i$ of learner $s_i$ will be output after training the diagnoser (i.e. fitting Eq.(\ref{equ:Camilla-Base-2})) , where each dimension of $A_i$ indicates the learner proficiency on specific skill. Then, we can obtain the overall \emph{Ability} $a_i$ of $s_i$ on dataset $E$ by
\begin{equation}
    a_i = \frac{1}{|E|}\sum\nolimits_{e_j\in E} \frac{Q_j \cdot A_i}{\sum\nolimits_{k=1}^K Q_{jk}} ,
\end{equation}
where $a_i \in [0, 1]$, $A_i \in \mathbb{R}^{1\times K}$, and $\sum\nolimits_{k=1}^K Q_{jk}$ is the number of explicit skills of sample $e_j$.


% \noindent\emph{Camilla.}~After training \emph{Camilla}, the vector of learner \emph{Ability} $A_i^{'}\in (0, 1)^{1\times K^{'}}$ is output as the assessment result of machine learning algorithm $s_i$, which denotes the proficiency of $s_i$ in these multiple facet skills. This original $A_i$ can also help us estimate the specific proficiency from $s_i$ to any single or subset of samples even if the sample-skill matrix $Q$ is implicitly defined as latent factors (i.e. both the meaning of each skill and the sample-skill relation is unknown). As shown in Figure~\ref{Fig.compare}, with the trained \emph{skill mask} factor, the \emph{Ability} $a_{\breve{E}}^i$ which summarizes the overall proficiency in a group of samples $\breve{E} \subseteq E$ is computed by:
% \begin{equation}
%     \begin{split}
%     \overline{A_i} &= \frac{1}{|\breve{E}|}\sum\nolimits_{e_j\in \breve{E}} Q_j^{'} \otimes A_i^{'}, \\
%     a_{\breve{E}}^i &= \sum\nolimits_{k=1}^{K^{'}}\overline{A_{ik}},
%     \end{split}
%     \label{output}
% \end{equation}
% where $Q_j^{'}$ is the \emph{skill mask} factor of sample $e_j$, $\otimes$ is element-product. $\overline{A_i} \in (0, 1)^{1\times K^{'}}$ denotes the aggregated \emph{Ability} weighted by sample \emph{skill mask} factors.

\noindent\emph{Camilla.}~After training \emph{Camilla} (e.g. fitting Eq.(\ref{equ:Camilla})), the vector of learner \emph{Ability} $A_i^{'}\in [0, 1]^{1\times K^{'}}$ is output as the assessment result of machine learning algorithm $s_i$ on multiple skills. This original $A_i$ can also help us estimate the specific proficiency from $s_i$ to any single or subset of samples even if the sample-skill matrix $Q$ is implicitly defined as latent factors (i.e. both the meaning of each skill and the sample-skill relation is unknown). As shown in Figure~\ref{Fig.compare}, to output the learner $s_i$'s ability $a_{\breve{E}}^i$ on a specific subset $\breve{E} \subseteq E$ of data samples, we first derive the overall \emph{skill mask} factor of the subset $Q_{\breve{E}}$ by averaging the \emph{skill mask} factors of the samples in this subset: 
\begin{equation}
    Q_{\breve{E}} = \frac{1}{|\breve{E}|}\sum\nolimits_{e_j\in \breve{E}} Q_j^{'}. 
\end{equation}
Then we summarize the overall ability ($a_{\breve{E}}^i$) of learner $s_i$ on the subset $\breve{E}$ of samples by summing the learner \emph{Ability} $A_i^{'}$ weighted by the \emph{skill mask} factor $Q_{\breve{E}}$:
\begin{equation}
a_{\breve{E}}^i = \sum\nolimits_{k=1}^{K^{'}}\overline{A_{ik}}, \quad \text{and} \quad
    \overline{A_i} = Q_{\breve{E}} \otimes A_i^{'},
\end{equation}
where $\otimes$ is element-product, and $\overline{A_i}$ is the learner \emph{Ability} scaled by $Q_{\breve{E}}$.

% \begin{equation}
%     \begin{split}
%     Q_{subset} &= \frac{1}{|\breve{E}|}\sum\nolimits_{e_j\in \breve{E}} Q_j^{'}, \\
%     a_{\breve{E}}^i &= \sum\nolimits_{k=1}^{K^{'}}\overline{A_{ik}},
%     \end{split}
%     \label{output}
% \end{equation}
% where $Q_j^{'}$ is the \emph{skill mask} factor of sample $e_j$, $\otimes$ is element-product. $\overline{A_i} \in (0, 1)^{1\times K^{'}}$ denotes the aggregated \emph{Ability} weighted by sample \emph{skill mask} factors.

Please note that the \emph{difficulty} factor $D_j^{'}$ of each sample $e_j$ in \emph{Camilla} is also a vector, and we can get the overall and unidimensional \emph{difficulty} of any sample similar to the way of computing $a_{\breve{E}}^i$, i.e. replacing $A_i^{'}$ by $D_j^{'}$ in Figure~\ref{Fig.compare}. 


\noindent\textbf{Implementation detail.}~\emph{hyperparameters.}
We consider a wide range of values for each hyperparameter of the \emph{Camilla}s through random search on each dataset. Specifically, the value set of each hyperparameter is considered as follows: 

~~ Learning rate~(LR) = [0.0001, 0.001, 0.005, 0.01],

~~ First Layer dimension in MLP~(LD1) = [16, 32, 64, 128, 256, 512],

~~ First Layer dimension in MLP~(LD2) = [16, 32, 64],

~~ Latent skill dimension~(LS) = [5, 10, 20, 50].


For all datasets, we split the response logs into the training set, validation set and test set as 6:2:2. We use the validation set to optimize the values of these hyperparameters in the \emph{reliability evaluation} experiment~(Table~\ref{Table. reliability}) with mini-batch size 256. We select the optimal architecture of \emph{Camilla}s and visualize the results in the other experiments: \emph{diagnostic factors interpretation}~(Figure~\ref{Fig. visualization1}, Figure~\ref{Fig. visualization2} and Figure~\ref{Fig. visualization3}), \emph{rank consistency}~(Figure~\ref{Fig.COR}a) and \emph{rank stability}~(Figure~\ref{Fig.COR}b). Table~\ref{Table: statistics} summarizes the statistics related to these datasets, and for more information about the learners please refer to Supplementary. 


\noindent\emph{ Architecture of Camilla.} The final hyperparameters and architectures of \emph{Camilla} for each dataset are as follows: 

~~\quad Dataset: \enspace\qquad\enspace LR, \quad LD1, \quad LD2, \quad LS

~~\quad Titanic: ~\qquad 0.001, ~\quad 128, ~~~\thinspace\quad 64, \quad\enspace 5

~~\quad CIFAR-100: ~\thinspace 0.001, ~\quad 128, ~~~\thinspace\quad 64, \quad\enspace 5

~~\quad ESOL: ~~\thinspace\thinspace\qquad 0.001, ~\quad\thinspace\thinspace\thinspace 64, ~~~\thinspace\quad 32,  \quad 10

~~\quad Diamond: ~\thinspace\quad 0.001, ~\quad\thinspace\thinspace\thinspace 32, ~~~\thinspace\quad 16, \quad\enspace 5

LD1 and LD2 refer to the dimensions of the first layer and the second layer in the MLP respectively. For reproducing our experimental results, we independently run each experiment for ten times and consider the following random seeds:

~~\quad Seed = [1, 21, 42, 84, 168, 336, 672, 1344, 2688, 5376]

For the \emph{diagnostic factor interpretation} experiments, we choose 42 as the seed, which is the answer to life, the universe and everything~\cite{sharifi2021out}.

We optimize the performance of \emph{Camilla-Base} and other baselines with same settings and same ranges of values with \emph{Camilla} whenever those values are applicable. For the implementations of IRT, MIRT, NeuralCD and MF, we use the public code at \href{https://github.com/bigdata-ustc/EduCDM}{https://github.com/bigdata-ustc/EduCDM}. All of those diagnosers are implemented by PyTorch, and we adopt the Adam optimizer~\cite{kingma2014adam} to optimize the parameters of all those diagnosers whenever applicable.


==> section/related_work.tex <==
\section*{Related Work}

\noindent  \textbf{Cognitive Diagnosis.} In psychometrics, cognitive diagnosis is developed to assess users' (e.g. students') proficiency on a set of tasks (e.g. exercises) or multiple skills through their interactive behaviors~(e.g. historical exercise records). According to different diagnostic goals, researchers designed the corresponding cognitive diagnosis models~(CDMs) with two components: (1)~the representations of latent cognitive states and (2)~the interactive function. Based on the way of modeling cognitive states, the mainstream CDMs can be generally divided into two categories: unidimension-oriented and multidimension-oriented. One prototype of the first type of CDMs is item response theory~(IRT)~\cite{lord1952theory, embretson2013item}, which characterizes students and exercises by a unidimensional variable respectively and predicts the probability that a student answers an exercise correctly as follows:
\begin{equation}
    P(r_{ij}=1|a_i, k_j, d_j) = \sigma(-1.7 k_j(a_i - d_j)),
    \label{equ:IRT}
\end{equation}
 where $a_i$ denotes the unidimensional \emph{Ability} (cognitive state) of student $i$, $k_j$ and $d_j$ represent the \emph{discrimination} and \emph{difficulty} of exercise $j$, and $\sigma$ is the Sigmoid function.

The other type of CDMs aims to diagnose the student proficiency on different skills. For instance, MIRT~\cite{reckase2009multidimensional} extends the $a_i$ and $k_j$ in IRT to multi-dimensional cognitive states. Also, Deterministic Input, Noisy ``And" gate model~(DINA)~\cite{de2009dina} describes each student with a binary vector that denotes whether the student masters a set of skills along with a Q-matrix which illustrates each exercise and relevant skills. Considering the limitations of the manually designed interaction functions of traditional CDMs (e.g. Eq.(\ref{equ:IRT})), NeuralCD~\cite{wang2020neural} combines deep neural networks to automatically learn such function. 
\begin{equation}
         x_{ij}=Q_j \circ\left(a_i-d_j\right) \times {k_j}, ~~
         P(y_{ij}=1) = \phi_n(...\phi_1(x_{ij})),
\end{equation}
 where $\circ$ is element-wise product and $Q_j$ denotes the skills related to exercise $j$. $\phi_n(...\phi_1)$ indicates multiple mapping layers. Capturing the connections between human learning and machine learning, in this paper, we aim to diagnose both unidimensional and multidimensional \emph{Ability} of machine learning algorithms with the help of psychometric theories from human measurement. However, existing CDMs cannot be directly applied due to the technical and domain challenges. For instance, the sample-skill relevancy (i.e. Q-matrix in psychometrics) is not always explicitly available in machine learning, in other words, we usually need to model the implicit skills for data samples. 
 
\noindent  \textbf{Existing Metrics and Interpretable Evaluation.} Currently, mainstream evaluation metrics generally adopt a rather simplistic unidimensional view of the machine learning algorithms, through summarizing their performance on single data samples. For better illustration, in the following we take the machine learning tasks of classification as example. In some typical and class-balanced classification datasets, such as CIFAR~\cite{cifar} and Imagenet~\cite{imagenet}, machine learning systems are ranked with Top-k \emph{Accuracy} classification score. While for the class-unbalanced classification tasks, mean average precision~(\emph{MAP}) and balanced \emph{F-score } are the widely used metrics. 

%  Considering the limitations of traditional coarse-grained metrics~\cite{japkowicz2006question, flach2019performance}, \textit{interpretable evaluation}~\cite{fu2020interpretable, narayanan2018humans, moraffah2020causal} aims at dividing the holistic performance of the algorithms into interpretable groups of samples. For instance, ExplainaBoard~\cite{liu2021explainaboard} annotates a large number of attributes of samples in different NLP tasks and fine-grained analyzes the performance of algorithms in different attributes. Similarly, Language Interpretability Tool~(LIT)~\cite{tenney2020language} provides visual explanations like attention weight and permits users real-time interact with machine learning algorithms to enable rapid error analysis. Different from existing solutions, our study is directly inspired by the psychometric theories, and we can collaboratively quantify both the multi-dimensional abilities of different algorithms and some of the sample factors (e.g. sample \emph{difficulty}) in a general way.

Considering the limitations of traditional coarse-grained metrics~\cite{japkowicz2006question, flach2019performance}, some general \textit{interpretable evaluation} research~\cite{fu2020interpretable, moraffah2020causal} aims at dividing the holistic performance of the algorithms into interpretable groups of samples. For instance, ExplainaBoard~\cite{liu2021explainaboard} annotates a large number of attributes of samples in different NLP tasks and fine-grained analyzes the performance of algorithms in different attributes. In addition, inspired by human Theory of Mind, some approaches~\cite{rabinowitz2018machine, cuzzolin2020knowing} seek to build a system to model agents' charateristics and mental states by predicting their future behaviour, particularly in \emph{Reinforcement Learning}~(RL) field. Different from these solutions, our study is directly inspired by the psychometric theories, and we can collaboratively quantify both the multi-dimensional abilities of different algorithms and some of the sample factors (e.g. sample \emph{difficulty}) in a general way.

Some other \emph{interpretable evaluation} methods~\cite{martinez2016making, martinez2019item} inspired by the psychometric theories predominantly utilize IRT as the backbone where the unidimensional metric can be applied in the evaluation of various machine learning tasks: question answering~\cite{rodriguez2021evaluation}, machine translation~\cite{hopkins-may-2013-models, otani-etal-2016-irt}, textual entailment~\cite{DBLP:conf/emnlp/LalorWY16, DBLP:conf/emnlp/LalorWY19}, chatbot evaluation~\cite{sedoc-ungar-2020-item} and AI video game~\cite{martinez2018dual} of RL. Rather than a simplistic unidimensional metric in IRT, our proposed framework aims at measure the multidimensional \emph{Ability} of different algorithms to better capture the pros and cons of each algorithm.

% Besides, \cite{martinez2018dual} use IRT to measure the performance of different agents on AI video game benchmarks.

%  \noindent \textbf{IRT in Machine Learning.} IRT has gained significant attention lately in machine learning research~\cite{martinez2016making, martinez2019item} where the unidimensional metric can be applied in the evaluation of various NLP tasks: question answering~\cite{rodriguez2021evaluation}, machine translation~\cite{hopkins-may-2013-models, otani-etal-2016-irt}, textual entailment~\cite{DBLP:conf/emnlp/LalorWY16, DBLP:conf/emnlp/LalorWY19} and chatbot evaluation~\cite{sedoc-ungar-2020-item}. Besides, \cite{martinez2018dual} use IRT to measure the performance of different agents on AI video game benchmarks. Furthermore, \cite{ensemble} ensembles multiple classifers to correctly classify hard instances by assigning different weights based on the diagnostic results of IRT. \cite{active} propose an active learning strategy measuring the information capacity of instances from the IRT-based function, which is prone to be more flexible in building transparent knowledge deep models. Rather than a simplistic unidimensional metric in IRT, Our proposed framework aims at measure the multidimensional \emph{Ability} of different algorithms to better capture the pros and cons of each algorithm.



